One-Shot Secure Aggregation: A Hybrid Cryptographic Protocol for Private Federated Learning in IoT

Federated Learning (FL) offers a promising approach to collaboratively train machine learning models without centralizing raw data, yet its scalability is often throttled by excessive communication overhead. This challenge is magnified in Internet of Things (IoT) environments, where devices face stringent bandwidth, latency, and energy constraints. Conventional secure aggregation protocols, while essential for protecting model updates, frequently require multiple interaction rounds, large payload sizes, and per-client costs rendering them impractical for many edge deployments. In this work, we present Hyb-Agg, a lightweight and communication-efficient secure aggregation protocol that integrates Multi-Key CKKS (MK-CKKS) homomorphic encryption with Elliptic Curve Diffie-Hellman (ECDH)-based additive masking. Hyb-Agg reduces the secure aggregation process to a single, non-interactive client-to-server transmission per round, ensuring that per-client communication remains constant regardless of the number of participants. This design eliminates partial decryption exchanges, preserves strong privacy under the RLWE, CDH, and random oracle assumptions, and maintains robustness against collusion by the server and up to $N-2$ clients. We implement and evaluate Hyb-Agg on both high-performance and resource-constrained devices, including a Raspberry Pi 4, demonstrating that it delivers sub-second execution times while achieving a constant communication expansion factor of approximately 12x over plaintext size. By directly addressing the communication bottleneck, Hyb-Agg enables scalable, privacy-preserving federated learning that is practical for real-world IoT deployments.

==> Threat-model.tex <==
\section{Threat Model}

In this section, we define the adversarial capabilities, the trust assumptions, and the security goals that our secure aggregation protocol must satisfy in the context of federated learning over IoT devices.

\subsection{Adversarial Capabilities}

We consider three classes of adversaries:

\begin{itemize}[leftmargin=*]
  \item \textbf{Honest-but-Curious Server.}  The central server \(S\) faithfully follows the protocol specification (key distribution, ciphertext aggregation, unmasking, etc.) but may record and analyze all messages it receives.  In particular, \(S\) sees the encrypted model updates \(\{c^i\}\) and the masked partial decryption shares \(\{\widetilde\mu_i\}\), and attempts to infer any client’s private update \(m_i\).
  \item \textbf{Honest-but-Curious Clients.}  A subset of clients may collude with \(S\) to share their own secret keys, ECDH-derived masks, or partial decryptions, in order to recover another client’s update.
  \item \textbf{External Eavesdropper.}  A network-level adversary who can intercept all messages exchanged between clients and server, but cannot modify or inject messages.  We assume all channels are authenticated and integrity-protected, so the eavesdropper cannot tamper with ciphertexts without detection.
\end{itemize}

\subsection{Trust Assumptions}

\begin{itemize}[leftmargin=*]
  \item \emph{Key Setup:}  We assume a common reference string (CRS) \(a\in\mathcal{R}_q\) is generated honestly once and shared with all parties.  
  \item \emph{Channel Authentication:}  Every client has an authenticated channel to the server (e.g.\ TLS) and can verify signatures on public keys.
  \item \emph{Honest Majority:}  At most \(k < N-1\) clients may collude with the server.  We require at least two non-colluding clients remain honest to ensure masks cancel correctly.
  \item \emph{Randomness:}  All parties sample their errors, masks, and ECDH exponents from the prescribed distributions (RLWE, ECDH) and do not leak this randomness.
\end{itemize}

\subsection{Security Goals}

Our protocol is designed to achieve the following properties against the above adversaries.

\begin{description}[leftmargin=*]
  \item[\textbf{Confidentiality.}]  
    No party (server or colluding clients) learns any individual client’s model update \(m_i\) in clear.  The server only learns the global sum \(\sum_i m_i\).
  \item[\textbf{Integrity.}]  
    The aggregated result computed by the server is guaranteed to be the exact arithmetic sum (modulo the plaintext modulus) of all honest clients’ plaintexts.  Malicious clients cannot distort the final sum without detection.
  \item[\textbf{Collusion Resistance.}]  
    Even if the server colludes with up to \(k \leq N-2\) clients, the updates of the remaining honest clients remain confidential.  The random masks introduced via ECDH+HKDF ensure no subset of fewer than \(N\) parties can unmask any single share.

\end{description}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse

\subsection{Definition}
- Server, Clients,Problems
- A figure
 (Secure FL, clients, server, how can we present to show that server needs only one round to obtain the final aggregation using CKKS)

 (Each Client i generates the key pair (pk, sk), Enc-pk-i))

\subsection{Security Requirements}
We consider two adversarial entities:
\begin{itemize}
    \item \textbf{Honest-but-Curious Server}: Follows protocol but attempts to infer client data from observed messages.
    \item \textbf{Honest-but-Curious Clients}: Subset of clients that collaborate to deduce others' private updates.
\end{itemize}

\subsection{Design Goal}

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
